DevSecOps in Robotics

Quality in software is often understood as "execution according to design purpose" whereas security means that "software will not put data or computing systems at risk of unauthorized access." There seems to be a connection between these two aspects but, how do we integrate both of them in the robotics development cycle? In this article we introduce DevSecOps in Robotics, a set of best practices designed to help roboticists implant security deep in the heart of their development and operations processes. First, we briefly describe DevOps, introduce the value added with DevSecOps and describe and illustrate how these practices may be implemented in the robotics field. We finalize with a discussion on the relationship between security, quality and safety, open problems and future research questions.

==> DevSecOps in Robotics/diagram/sequence_diagram_aztarna.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{1.8}
	\newinst{Robot}{Robot target}
	\newinst[10.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	
    	\begin{sdblock}{Phase 1}{Scan and analyze}
        	%\stepcounter{seqlevel}
    		\begin{call}{Aztarna}{}{Robot}{}
    		\end{call}
	    \end{sdblock}
	
	    \begin{sdblock}{Phase 2} {Footprint}
	        %\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{}{Robot}{}
        	\end{call}
        \end{sdblock}		    

	    \begin{sdblock}{Phase 3} {Fingerprint (outside of the scope)}
	        %\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{}{Robot}{}
        	\end{call}

    	\end{sdblock}	
	          
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of \texttt{aztarna}.}
 \label{fig:aztarna/general}
\end{figure}

==> DevSecOps in Robotics/diagram/sequence_diagram_aztarna_industrialrouters.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Router}{Industrial router target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan and identification}
        	\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{HTTP Request}{Robot}{HTTP Response containing headers}
        	\end{call}
	    \end{sdblock}
	    \begin{sdblock}{Phase 2}{Authentication}
	        \stepcounter{seqlevel}
	        \begin{call}
	        {Aztarna}{HTTP Request}{Robot}{HTTP 401 Unauthorized response}
	        \end{call}
	        \begin{call}
	        {Aztarna}{HTTP basic authentication response}{Robot}{HTTP 200 OK Response}
	        \end{call}
	        
	        
	    \end{sdblock}
         
	%\begin{sdblock}{alt}{$S$ chooses TCPROS}	
	%\mess{Subscriber}{Terminate connection}{Publisher}
	%	\begin{call}{Subscriber}{Subscribe}{Aztarna}{}
	%	\end{call}
	%	\stepcounter{seqlevel}
	%	\mess{Aztarna}{False data}{Subscriber}
	%\end{sdblock}
	%\begin{sdblock}{Phase 2b}{$sub$ w"ahlt UDPROS als Transportprotokoll}
	          
   \end{scope}
\end{sequencediagram}
 \label{fig:aztarna/industrial_routers}
 \caption{\texttt{aztarna} performing identification and authentication phases for an industrial router.}
\end{figure}

==> DevSecOps in Robotics/diagram/sequence_diagram_aztarna_ros.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Robot}{Robot target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan and analyze}
    	\stepcounter{seqlevel}
		\begin{call}{Aztarna}{Invoke \texttt{getsystemstate()}}{Robot}{Return basic footprint}
		\end{call}
		
	\end{sdblock}
	\begin{sdblock}{Phase 2} {Footprint}	

	\begin{sdblock}{Node 1} {}
    	\begin{call}{Aztarna}{Fetch nodes URI through     \texttt{lookupNodes()}}{Robot}{}
    	\end{call}
        
        \begin{call}{Aztarna}{Fetch list of topics through \texttt{getTopicTypes()}}{Robot}{}
    	\end{call}
    	
	\end{sdblock}

	\begin{sdblock}{Node N} {}
    	\begin{call}{Aztarna}{Fetch nodes URI through     \texttt{lookupNodes()}}{Robot}{}
    	\end{call}
        
        \begin{call}{Aztarna}{Fetch list of topics through \texttt{getTopicTypes()}}{Robot}{}
    	\end{call}
    	
	\end{sdblock}	
         
	%\begin{sdblock}{alt}{$S$ chooses TCPROS}	
	%\mess{Subscriber}{Terminate connection}{Publisher}
	%	\begin{call}{Subscriber}{Subscribe}{Aztarna}{}
	%	\end{call}
	%	\stepcounter{seqlevel}
	%	\mess{Aztarna}{False data}{Subscriber}
	%\end{sdblock}
	%\begin{sdblock}{Phase 2b}{$sub$ w"ahlt UDPROS als Transportprotokoll}
	          
   \end{sdblock}		
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of a \texttt{aztarna} scanning a ROS target.}
 \label{fig:aztarna/ros}
\end{figure}

==> DevSecOps in Robotics/diagram/sequence_diagram_aztarna_sros.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Robot}{Robot target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan}
    	\stepcounter{seqlevel}
		\mess{Aztarna}{Client Hello}{Robot}{Server Hello}
	\end{sdblock}
	\begin{sdblock}{Phase 2}{Fingerprinting}
		\mess{Robot}{Server Certificate}{Aztarna}
		\mess{Robot}{Client Certificate Request}{Aztarna}
		\mess{Robot}{Server Hello Done}{Aztarna}
	\end{sdblock}
	\begin{sdblock}{Phase 2}{Close Connection}
		\mess{Aztarna}{Disconnect TCP session}{Robot}
	\end{sdblock}
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of a \texttt{aztarna} performing the scan and fingerprinting phases for SROS.}
 \label{fig:aztarna/sros}
\end{figure}

==> diagram/sequence_diagram_aztarna.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{1.8}
	\newinst{Robot}{Robot target}
	\newinst[10.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	
    	\begin{sdblock}{Phase 1}{Scan and analyze}
        	%\stepcounter{seqlevel}
    		\begin{call}{Aztarna}{}{Robot}{}
    		\end{call}
	    \end{sdblock}
	
	    \begin{sdblock}{Phase 2} {Footprint}
	        %\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{}{Robot}{}
        	\end{call}
        \end{sdblock}		    

	    \begin{sdblock}{Phase 3} {Fingerprint (outside of the scope)}
	        %\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{}{Robot}{}
        	\end{call}

    	\end{sdblock}	
	          
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of \texttt{aztarna}.}
 \label{fig:aztarna/general}
\end{figure}

==> diagram/sequence_diagram_aztarna_industrialrouters.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Router}{Industrial router target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan and identification}
        	\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{HTTP Request}{Robot}{HTTP Response containing headers}
        	\end{call}
	    \end{sdblock}
	    \begin{sdblock}{Phase 2}{Authentication}
	        \stepcounter{seqlevel}
	        \begin{call}
	        {Aztarna}{HTTP Request}{Robot}{HTTP 401 Unauthorized response}
	        \end{call}
	        \begin{call}
	        {Aztarna}{HTTP basic authentication response}{Robot}{HTTP 200 OK Response}
	        \end{call}
	        
	        
	    \end{sdblock}
         
	%\begin{sdblock}{alt}{$S$ chooses TCPROS}	
	%\mess{Subscriber}{Terminate connection}{Publisher}
	%	\begin{call}{Subscriber}{Subscribe}{Aztarna}{}
	%	\end{call}
	%	\stepcounter{seqlevel}
	%	\mess{Aztarna}{False data}{Subscriber}
	%\end{sdblock}
	%\begin{sdblock}{Phase 2b}{$sub$ w"ahlt UDPROS als Transportprotokoll}
	          
   \end{scope}
\end{sequencediagram}
 \label{fig:aztarna/industrial_routers}
 \caption{\texttt{aztarna} performing identification and authentication phases for an industrial router.}
\end{figure}

==> diagram/sequence_diagram_aztarna_ros.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Robot}{Robot target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan and analyze}
    	\stepcounter{seqlevel}
		\begin{call}{Aztarna}{Invoke \texttt{getsystemstate()}}{Robot}{Return basic footprint}
		\end{call}
		
	\end{sdblock}
	\begin{sdblock}{Phase 2} {Footprint}	

	\begin{sdblock}{Node 1} {}
    	\begin{call}{Aztarna}{Fetch nodes URI through     \texttt{lookupNodes()}}{Robot}{}
    	\end{call}
        
        \begin{call}{Aztarna}{Fetch list of topics through \texttt{getTopicTypes()}}{Robot}{}
    	\end{call}
    	
	\end{sdblock}

	\begin{sdblock}{Node N} {}
    	\begin{call}{Aztarna}{Fetch nodes URI through     \texttt{lookupNodes()}}{Robot}{}
    	\end{call}
        
        \begin{call}{Aztarna}{Fetch list of topics through \texttt{getTopicTypes()}}{Robot}{}
    	\end{call}
    	
	\end{sdblock}	
         
	%\begin{sdblock}{alt}{$S$ chooses TCPROS}	
	%\mess{Subscriber}{Terminate connection}{Publisher}
	%	\begin{call}{Subscriber}{Subscribe}{Aztarna}{}
	%	\end{call}
	%	\stepcounter{seqlevel}
	%	\mess{Aztarna}{False data}{Subscriber}
	%\end{sdblock}
	%\begin{sdblock}{Phase 2b}{$sub$ w"ahlt UDPROS als Transportprotokoll}
	          
   \end{sdblock}		
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of a \texttt{aztarna} scanning a ROS target.}
 \label{fig:aztarna/ros}
\end{figure}

==> diagram/sequence_diagram_aztarna_sros.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Robot}{Robot target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan}
    	\stepcounter{seqlevel}
		\mess{Aztarna}{Client Hello}{Robot}{Server Hello}
	\end{sdblock}
	\begin{sdblock}{Phase 2}{Fingerprinting}
		\mess{Robot}{Server Certificate}{Aztarna}
		\mess{Robot}{Client Certificate Request}{Aztarna}
		\mess{Robot}{Server Hello Done}{Aztarna}
	\end{sdblock}
	\begin{sdblock}{Phase 2}{Close Connection}
		\mess{Aztarna}{Disconnect TCP session}{Robot}
	\end{sdblock}
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of a \texttt{aztarna} performing the scan and fingerprinting phases for SROS.}
 \label{fig:aztarna/sros}
\end{figure}
